Symmetric Strategies for Multi-Access IoT Network Optimization: A Common Information Approach

In the context of IoT deployments, a multitude of devices concurrently require network access to transmit data over a shared communication channel. Employing symmetric strategies can effectively facilitate the collaborative use of the communication medium among these devices. By adopting such strategies, devices collectively optimize their transmission parameters, resulting in minimized collisions and enhanced overall network throughput. Our primary focus centers on the formulation of symmetric (i.e., identical) strategies for the sensors, aiming to optimize a finite horizon team objective. The imposition of symmetric strategies introduces novel facets and complexities into the team problem. To address this, we embrace the common information approach and adapt it to accommodate the use of symmetric strategies. This adaptation yields a dynamic programming framework grounded in common information, wherein each step entails the minimization of a single function mapping from an agent's private information space to the space of probability distributions over possible actions. Our proposed policy/method incurs a reduced cumulative cost compared to other methods employing symmetric strategies, a point substantiated by our simulation results.

==> name.tex <==
#!/usr/bin/env python3
from dotenv import load_dotenv
from langchain.chains import RetrievalQA
from langchain.embeddings import HuggingFaceEmbeddings
from langchain.callbacks.streaming_stdout import StreamingStdOutCallbackHandler
from langchain.vectorstores import Chroma
from langchain.llms import GPT4All, LlamaCpp
import os
import time
import csv
from colorama import Fore, Back, Style
from colorama import init as colorama_init
from constants import CHROMA_SETTINGS

colorama_init(autoreset=True)
load_dotenv()

embeddings_model_name = os.environ.get("EMBEDDINGS_MODEL_NAME")
persist_directory = os.environ.get('PERSIST_DIRECTORY')
embedding_model_directory = os.environ.get('EMBEDDING_DIRECTORY')
model_type = os.environ.get('MODEL_TYPE')
model_path = os.environ.get('MODEL_PATH')
model_n_ctx = os.environ.get('MODEL_N_CTX')
model_n_batch = int(os.environ.get('MODEL_N_BATCH', 8))
target_source_chunks = int(os.environ.get('TARGET_SOURCE_CHUNKS', 4))
temperature = os.environ.get('TEMPERATURE')
n_gpu_layers = 43


def main():
    # Parse the command line arguments
    embeddings = HuggingFaceEmbeddings(model_name=embeddings_model_name, cache_folder=embedding_model_directory)
    db = Chroma(persist_directory=persist_directory, embedding_function=embeddings, client_settings=CHROMA_SETTINGS)
    retriever = db.as_retriever(search_kwargs={"k": target_source_chunks})
    callbacks = [StreamingStdOutCallbackHandler()]
    # Prepare the LLM
    if model_type=="LlamaCpp":
        llm = LlamaCpp(
		model_path=model_path,
		temperature =temperature,
		n_gpu_layers=n_gpu_layers,
		n_batch=model_n_batch,
		n_ctx = 2048,
		max_tokens = 2000,
		top_p = 1,
	 	callbacks=callbacks,
		verbose=True
		)
    elif model_type=="GPT4All":
        llm = GPT4All(model=model_path, max_tokens=model_n_ctx, backend='gptj', n_batch=model_n_batch,
                          callbacks=callbacks, verbose=False)
    else:
	# raise exception if model_type is not supported
        raise Exception(f"Model type {model_type} is not supported. Please choose one of the following: LlamaCpp, GPT4All")

    qa = RetrievalQA.from_chain_type(llm=llm, chain_type="stuff", retriever=retriever, return_source_documents=True)
    
    def initialize_csv_file():
        if not os.path.isfile("output.csv"):
            with open("output.csv",mode="w", newline="") as file:
                writer=csv.writer(file)
                writer.writerow(["Query", "Response", "Processing Time (seconds)"])
    
         
    # Interactive questions and answers
    while True:
        query = input("\nEnter a query: ")
        if query == "exit":
            break
        if query.strip() == "":
            continue
        initialize_csv_file()
        # Get the answer from the chain
        start = time.time()
        res = qa(query)
        answer, docs = res['result'], res['source_documents']
        end = time.time()
        proc_time = round(end - start, 2)
        # Print the result
        print(Fore.WHITE + Style.BRIGHT + "\n\n> Question:")
        print(Fore.WHITE + Style.BRIGHT + f"{query}")
        print(Fore.CYAN + Style.BRIGHT + f"\n> Answer (took {round(end - start, 2)} s.):")
        print(Fore.CYAN + Style.BRIGHT + f"{answer}")

        # Print the relevant sources used for the answer
        for document in docs:
            print(Fore.GREEN + Style.BRIGHT + "\n> " + f'{document.metadata["source"]}' + ":")
            print(Fore.YELLOW + Style.BRIGHT + f"{document.page_content}")
            
            with open("output.csv",mode="a",newline="") as file:
                writer=csv.writer(file)
                writer.writerow([query, answer, proc_time,document.metadata["source"],document.page_content])  


if __name__ == "__main__":
    main()


    qa = RetrievalQA.from_chain_type(llm=llm, chain_type="stuff", retriever=retriever, return_source_documents=True)
    # Interactive questions and answers
    while True:
        query = input("\nEnter a query: ")
        if query == "exit":
            break
        if query.strip() == "":
            continue

        # Get the answer from the chain
        start = time.time()
        docs1=retriever.get_relevant_documents(query)
        for doc in [document.metadata["source"] for document in docs1]:
            if doc.split(".")[-1] in ['csv']:
                print("One of the document is a csv file I should use Python REPL")
                print(doc)
                df = pd.read_csv(doc)
                agent=create_pandas_dataframe_agent(llm,df,verbose=True)
                resp=agent.run(query)
                answer=resp['result']
                
            else:
                res = qa(query)
                answer, docs = res['result'], res['source_documents']
        
        
        end = time.time()





from langchain.agents import create_pandas_dataframe_agent
from langchain.llms import GPT4All, LlamaCpp
from langchain.agents.agent_types import AgentType
from langchain.callbacks.streaming_stdout import StreamingStdOutCallbackHandler

import pandas as pd

df=pd.read_csv(r"C:/Users/e191420/Llama_CSV/titanic_csv")
llm=LlamaCpp(model_path=r'C:\Users\e191420\Llama_CSV\models\llama-2-13b-chat.ggmlv3.q4_0.bin',temperature=0.0, n_ctx=1024)
agent=create_pandas_dataframe_agent(llm,df,verbose=True)
agent.run("How many rows are there?")
agent.run("How many people have more than 3 siblings?")


def dataframe_loader(paths, query):
    def dataframe_query_constructor(paths: list):
        constructor = []
        for i, path in enumerate(paths, start=1):
            ext = path.split(".")[-1]
            if ext.lower() == "csv":
                df = pd.read_csv(path)
            elif ext.lower() in ["xls","xlsx"]:
                df = pd.read_excel(path)
            else:
                raise TypeError("file is not a dataframe")
            constructor.append(f"```python\nprint(df{i}.head())\n```")
            constructor.append(f"```output\n{df.head()}\n```")
            constructor.append(f"```python\nprint(df{i}.columns.tolist())\n```")
            constructor.append(f"```output\n{df.columns.tolist()}\n```")
        return "\n".join(constructor)

    TEMPLATE = textwrap.dedent(f"""\
You are working with multiple pandas dataframes in Python. 
These are the dataframes you will be working with:
{dataframe_query_constructor(paths)}

Answer this question using pandas operations.
Don't assume anything. Use dataframe operations to ensure the answer is correct.

Query: {query}
Answer:
```python
print(""")

    return TEMPLATE
